Locally Phase-Engineered MoTe$_2$ for Near-Infrared Photodetectors

Transition metal dichalcogenides (TMDs) are ideal systems for two-dimensional (2D) optoelectronic applications, owing to their strong light-matter interaction and various band gap energies. New techniques to modify the crystallographic phase of TMDs have recently been discovered, allowing the creation of lateral heterostructures and the design of all-2D circuitry. Thus far, the potential benefits of phase-engineered TMD devices for optoelectronic applications are still largely unexplored. The dominant mechanisms involved in the photocurrent generation in these systems remain unclear, hindering further development of new all-2D optoelectronic devices. Here, we fabricate locally phase-engineered MoTe$_{2}$ optoelectronic devices, creating a metal (1T') semiconductor (2H) lateral junction and unveil the main mechanisms at play for photocurrent generation. We find that the photocurrent originates from the 1T'-2H junction, with a maximum at the 2H MoTe$_{2}$ side of the junction. This observation, together with the non-linear IV-curve, indicates that the photovoltaic effect plays a major role on the photon-to-charge current conversion in these systems. Additionally, the 1T'-2H MoTe$_{2}$ heterojunction device exhibits a fast optoelectronic response over a wavelength range of 700 nm to 1100 nm, with a rise and fall times of 113 $\mu$s and 110 $\mu$s, two orders of magnitude faster when compared to a directly contacted 2H MoTe$_{2}$ device. These results show the potential of local phase-engineering for all-2D optoelectronic circuitry.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
